Inequalities and tail bounds for elementary symmetric polynomial with applications

We study the extent of independence needed to approximate the product of bounded random variables in expectation, a natural question that has applications in pseudorandomness and min-wise independent hashing. For random variables whose absolute value is bounded by $1$, we give an error bound of the form $\sigma^{\Omega(k)}$ where $k$ is the amount of independence and $\sigma^2$ is the total variance of the sum. Previously known bounds only applied in more restricted settings, and were quanitively weaker. We use this to give a simpler and more modular analysis of a construction of min-wise independent hash functions and pseudorandom generators for combinatorial rectangles due to Gopalan et al., which also slightly improves their seed-length. Our proof relies on a new analytic inequality for the elementary symmetric polynomials $S_k(x)$ for $x \in \mathbb{R}^n$ which we believe to be of independent interest. We show that if $|S_k(x)|,|S_{k+1}(x)|$ are small relative to $|S_{k-1}(x)|$ for some $k>0$ then $|S_\ell(x)|$ is also small for all $\ell > k$. From these, we derive tail bounds for the elementary symmetric polynomials when the inputs are only $k$-wise independent.

==> intro.tex <==
\section{Introduction}

In this work, we consider a natural question in probability, which has many application in computer science (\cite{Indyk,EGNLV,GMRTV}): {\em Let $X_1,\ldots,X_n$ be random variables each distributed in the range $[0,1]$. What is the smallest
value of $k = k(\delta)$ such that whenever the $X_i$s are sampled according to a $k$-wise independent
distribution $\D$, }
\begin{align}
\label{eq:k-wise}
\left|\E_\D[\prod_{i=1}^n X_i] - \prod_{i=1}^n\mu_i \right| \leq \delta. 
\end{align}
Note that if the $X_i$s are truly independent, then the LHS is $0$.

The results of \cite{EGNLV,Indyk} tell us that $k = O(\log(1/\delta)$
suffices. They prove this by using the inclusion/exclusion
priniciple (or equivalently the Bonferroni inequalities), and bounding
its error using the classical Maclaurin identities for elementary symmetric polynomials.

In this work, we propose an alternate approach which gives an improved
bound in the setting where the $X_i$s have small variance relative to
their mean-squared. More precisely, if
\[ \sigma^2 = \sum_{i=1}^n\frac{\sigma_i^2}{\mu_i^2} < 1 \]
we show that $k = O(\log(1/\delta)/\log(1/\sigma))$-wise
indepenendence suffices for Equation \eqref{eq:k-wise} to
hold. Concretely, in the setting where $\sigma^2 < n^{-c}$ for some $c
>0$, we show that $O(1)$-wise indepenendence suffices to achieve
polynomially small error in Equation \eqref{eq:k-wise}, as opposed to
$O(\log(n))$-wise independnece. 

Our motivation for considering this problem comes from a recent
construction of pseudorandom genaerators for combinatorial rectangles
due to \cite{GMRTV}. This is an important
problem in the construction of explicit pseudorandom
generators whcih has been studied intensively over the last two
decades  \cite{}. Such generators are known to imply small families of
min-wise independent permutations \cite{}. Using our approach above, we give an analysis of the PRG
function construction of \cite{GMRTV} from the viewpoint of hash
function. Our analysis is simpler and more modular, and also improves
the seed-length of the construction in lower order
terms. Given the fundamental nature of the question, we believe our
results will find other applications in pseudorandomness. 

The novel technical ingredient in our analysis is a new analytic inequality about 
symmetric polynomials in real variables which we believe is
independently interesting.  The elementary symmetric polynomials are a basic family of functions
that are invariant under any permutation of the inputs.
The $k$'th symmetric polynomial is defined as\footnote{We omit
the dependence on $n$ from the notation. It is clear from the context.
The polynomial $S_0$ is defined to be $1$.} 
$$S_k(a) =   \sum_{T \subseteq [n]: |T|=k} \prod_{i \in T} a_i$$
for all $a = (a_1,a_2,\ldots,a_n)$.
We show that for any real vector $z$, if $|S_k(z)|,|S_{k+1}(z)|$ are
small relative to $|S_{k-1}(z)|$ for some $k>0$, then $|S_\ell(z)|$ is
also small for all $\ell > k$.  

In what follows, we give an overview of the new inequality, its use in the
derivation of sharp tail bounds for elementary symmetric polynomilas
under limited independence and finally the application of these bounds
the the construction of pseudrandom generators/hash functions. 

\subsection{An inequality for elementary symmetric polynomials}

The $k^{th}$ elementary polynomial is defined as
\[ S_k(a) =   \sum_{T \subseteq [n]: |T|=k} \prod_{i \in T} a_i \]
for all $a = (a_1,a_2,\ldots,a_n) \in \R^n$. 
They appear as coefficients of a 
univariate polynomial with roots $-a_1,\ldots,-a_n \in \R$. That is,
$$\prod_{i \in [n]} (\xi + a_i) = \sum_{k=0}^n \xi^k S_{n-k}(a).$$

This work focuses on their growth rates. Specifically, we study how local information on $S_k(a)$
for two consecutive values of $k$ implies global information for all larger values of $k$.
Inequalities in these polynomials have been studied in
mathematics, dating back to classical results of Newton and
Maclaurin (see \cite{CS} for a survey of such inequalities).

An interesting property over the real numbers is
that if $p(\xi)$ is a real univariate polynomial
of degree $n$ with $n$ nonzero roots 
and $p'(0) = p''(0) = 0$ then $p \equiv 0$.
%previously:
%monic polynomial of degree $n$ with $n$ real roots
%is such that $p'(0) = p''(0) = 0$ then $p(\xi) = \xi^n$.
%this is wrong e.g. $\xi^2(x-1)$
This follows by simple properties of the symmetric
polynomials over the real numbers: 
We may write
\begin{align}
\label{eqn:propOfSk}
p(\xi) = \prod_{i \in [n]} (\xi b_i + 1) = \sum_{k=0}^n \xi^k S_k(b).
\end{align}
The condition on the derivatives of $p$
is equivalent to $S_1(b) = S_2(b) = 0$,
and the following fact completes the argument.
\begin{fact} 
\label{fact;1}
Over the real numbers, if $S_1(b)=S_2(b) = 0$ then $b=0$.
\end{fact}
%which implies
%over the real numbers that $b = 0$.
This does not hold over all fields,
for example, the polynomial $p(\xi) = \xi^3+1$ is of degree three, has three nonzero 
complex roots and $p'(0) = p''(0) = 0$. 

A robust version of Fact~\ref{fact;1} was recently proved in \cite{GMRTV}:
%\begin{theorem}
%\label{thm:GMRTV}
%There is a constant $c$ such that
%\Anote{changed presentation a bit--due to Avi's comment.} 
For every $a \in \R^n$ and $k \in [n]$,
\begin{align}
\label{eqn:GMR}
 |S_k(a)| \leq  \left(S^2_1(a) + 2|S_2(a)|\right)^{k/2} .
\end{align}
%\end{theorem}
That is, if $S_1(a),S_{2}(a)$ are small in absolute value, then so is
everything that follows. We provide an essentially optimal bound.

\begin{theorem}
\label{thm:boundUsingS1E2}
For every $a \in \R^n$ and $k \in [n]$,
\[ |S_k(a)| \leq  \left(\frac{6 e (S^2_1(a) + |S_2(a)|)^{1/2}}{k^{1/2} }\right)^k .\]
\end{theorem}

The parameters promised by Theorem~\ref{thm:boundUsingS1E2} are tight up to an exponential in $k$
which is often too small to matter
(we do not attempt to optimise the constants).
For example, if $a_i = (-1)^i$
for all $i  \in [n]$ then
$|S_1(a)| \leq 1$ and $|S_2(a)| \leq n+1$
but
$S_k(a)$ is roughly $(n/k)^{k/2}$.

The argument is quite general, and similar bounds may be obtained for functions that are recursively
defined. Our proof is analytic and uses the method of Lagrange multipliers, and is
different from that of \cite{GMRTV} which relied on the
Newton-Girrard identities.
\XX{The proof can be found in Section~\ref{sec:inequalities}.}

Stronger bounds are known when the inputs are nonnegative.
When $a_i \geq 0$ for all $i \in [n]$, the classical Maclaurin inequalities \cite{CS} imply that
\begin{align*}
S_k(a) \leq \left(\frac{e}{k}\right)^k(S_1(a))^k .
\end{align*}
In contrast, when we do not assume non-negativity, one cannot hope for
such bounds to hold under the assumption that $|S_1(a)|$ or any single
$|S_k(a)|$ is small (cf.\ the alternating signs example above).


A more general statement than Fact~\ref{fact;1} actually holds (see
Appendix \ref{app:proof} for a proof).
\begin{fact}
\label{fact:2}
Over the reals, if $S_k(a) = S_{k+1}(a) = 0$ for $k > 0$
then $S_\ell(a) =0$ for all $\ell \geq k$. 
\end{fact}
We prove a robust version of this fact as well:
A twice-in-a-row bound on the increase of the symmetric functions
implies a bound on what follows.

\begin{theorem}
\label{thm:GenBound}
For every $a \in \R^n$, if $S_k(a) \neq 0$ 
and 
\begin{align*}
\left|{k+1 \choose k}\frac{S_{k+1}(a)}{S_k(a)} \right| & \leq C
\ \ \text{and} \ \
\left| {k+2 \choose k}\frac{S_{k+2}(a)}{S_{k}(a)} \right| \leq
C^2
\end{align*}
then for every $1 \leq h \leq n -k$,
\begin{align*}
\left|{ k + h \choose k} \frac{S_{k+ h}(a)}{S_k(a)}\right| \leq \left(\frac{6eC}{h^{1/2}}\right)^h .
\end{align*}
\end{theorem}

\XX{The proof of Theorem~\ref{thm:GenBound}
is by reduction to Theorem~\ref{thm:boundUsingS1E2}.
In a nutshell,
it is carried by applying
Theorem~\ref{thm:boundUsingS1E2}
to the $k$'th derivative of the polynomial defined in Equation \eqref{thm:boundUsingS1E2}.
The proof can be found at the end of Section~\ref{sec:inequalities}.}



\subsection{Tail bounds under limited independence}

Pseudorandomness studies the possibility of removing randomness
from randomized algorithms while maintaining functionality.
A central notion in this study is $t$-wise independence.
The $n$ random variables $X_1,\ldots,X_n$ are $t$-wise
independent if every subset of $k$ of them are independent.
It turns out that one may produce $t$-wise independent distributions
using much fewer bits than are required for producing a fully independent distribution \cite{ABI,CG}, and this is of course useful for derandomization.

The authors of \cite{GMRTV} used this idea to construct pseudorandom generators
for several families of tests including read-once DNF formulas and
combinatorial rectangles. A key part of their proof was to show that
the expected value of 
$\prod_{i \in [n]}(1+X_i)$
does not significantly change
between the case the inputs are independent and
the case the inputs are only $t$-wise independent,
under the assumption that $\E[X_i] =0$ for all $i \in [n]$ and $\sum_i\Var[X_i] \ll 1$. 

One approach to control the behaviour of 
$\prod_{i \in [n]}(1+X_i)$
is taking logarithms and using known concentration bounds
for sums of independent random variables. 
What happens, however, in settings where  
$X_i$ may take the value $-1$ or large positive values, 
when there is no good approximation to $\ln(1 + X_i)$? 
Such settings arise for example in the analysis
of the pseudorandom generators \cite{GMRTV}. 
Even assuming that $X_i$ is nicely bounded, and $\ln(1 + X_i)$ is well
approximated by the Taylor series, analyzing the error seems to require
higher moment bounds for the individual $X_i$s.
%
%
%\footnote{Used to be: to control $\prod_{i \in [n]} (1+X_i)$,
%we would need strong concentration bounds for $\sum_{i \in [n]} X_i$. But our alternate approach shows that this is not true? This is only an artifact of taking logs}


  
An alternate approach adopted in \cite{GMRTV} is to observe that
$$\prod_{i \in [n]}(1+X_i) = \sum_{\ell=0}^n S_\ell(X_1,\ldots,X_n),$$
and try to get a better control by understanding the behavior of the symmetric polynomials. 
A key ingredient of \cite{GMRTV} is indeed about controlling 
$$\sum_{\ell = k}^n |S_\ell(X_1,\ldots,X_n)|,$$
assuming the distribution is $O(k)$-wise independent. 
Potentially, this approach
does not require any boundedness assumptions,
and it could also work without higher moment estimates since all the polynomials involved are multilinear. 
%At a high level, this is because the $S_k$s being multilinear are less
%sensitive to a few large values in the $X_i$s, as opposed to $(\sum_i
%X_i)^k$. 
\XX{
Nevertheless, the results of \cite{GMRTV} did require controlling higher moments of the $X_i$s as well. 
The reason is that they did not have an analogue of Theorem \ref{thm:GenBound}. So in order to use Equation \eqref{eqn:GMR}, they still
needed {\em strong} concentration for $S_1$ and $S_2$ which they obtained by bounding the higher moments. 
%This again requires higher moment bounds on individual variables.
Our result removes the need for higher moment bounds:
%We will make this precise 
%by showing that
we show that under $k$-wise independence, one can control the distribution of
$S_\ell(X_1,\ldots,X_n)$ even for $\ell > k$, given only first and second moment bounds on the individual $X_i$s.
}

Let $X =(X_1,\ldots,X_n)$ be a vector of real valued random variables so that
$$\E[X_i] = 0$$ for all $i \in [n]$, and denote
%Denote $\sigma_i^2 = \Var[X_i]$ for all $i \in [n]$, and   
\[\sigma^2 = \sum_{i \in [n]} \Var[X_i].\]  
Let $\cal{U}$ denote the distribution where the coordinates of $X$ are independent.
It is easy to show (see Lemma \ref{lem:exp-kwise}) that
\[ \E_{X \in \cal{U}}[|S_\ell(X)|] \leq \frac{\sigma^\ell}{\sqrt{\ell!}}.\]
In particular, if $\sigma^2 <1$ then $\E[|S_\ell|]$
decays exponentially with $\ell$.  For $t >0$ and $t\sigma
\leq 1/2$, we may also conclude (see Corollary \ref{cor:k-wise})
\begin{align}
\label{eq:tail}
\Pr_{X \in \cal{U}}\left[\sum_{\ell = k}^n |S_\ell(X)| \geq 2(t\sigma)^k\right]
\leq 2t^{-2k}.
\end{align}


Bounding $\E[|S_\ell|]$ for $\ell \leq k$ for more general $X$ 
only requires the distribution to be $(2k)$-wise
independent. It can be shown (see Section \ref{sec:lower}) that this is
  not enough to get strong bounds on $\E[|S_\ell|]$ for $\ell > 2k
  +1$. Nevertheless, we are able to show a tail bound which holds
  under limited independence, due to properties of the symmetric  polynomials.


\begin{theorem}
\label{thm:main}
Let $\cal{D}$ denote a distribution over $X = (X_1,\ldots,X_n)$
where $X_1,\ldots,X_n$ are $(2k+2)$-wise independent.
Assume $\E[X_i]=0$ for all $i \in [n]$,
and denote $\sigma = \sum_{i \in [n]} \Var[X_i]$. 
For $t >0$ and\footnote{A weaker but more technical assumption
on $t,\sigma,k$ suffices, see Equation \eqref{eqn:Endsum}.} $16 e t\sigma \leq 1$,
\begin{align}
\label{eq:kwise-tail2}
\Pr_{X \in \cal{D}} \left[\sum_{\ell=k}^n |S_\ell(X)| \geq 2(6 e t\sigma)^k \right] 
\leq 2t^{-2k} .
\end{align}
%and if we denote $p(x_1,\ldots,x_n) = \prod_{i \in [n]} (1+x_i)$
%then\footnote{Observe $\E_{X \in \cal{U}} [ p(X) ]=1$.}
%$$\Pr_{X \in \cal{D}} \left[ |p(X) - 1| \geq 2(6 e t\sigma)^k \right]
%\leq 2 t^{-2k}.$$
\end{theorem}


Comparing Equation \eqref{eq:kwise-tail2} to Equation \eqref{eq:tail} we see that it has a similar
asymptotic behaviour. A key ingredient in our proof is to show that although we
cannot upper bound the expectation of $|S_\ell|$ for large $\ell$ under
$k$-wise independence alone, we can still show good tail bounds for
it. Lemma~\ref{lem:main} below shows that for $t > 0$ and for $\ell \geq k$, the bounds
\[ |S_\ell(X)|  \leq (6 e t\sigma)^{\ell}  
\left( \frac{k}{\ell} \right)^{\ell/2} \]
hold except with $\cal{D}$-probability $2t^{-2k}$. 

In Section \ref{sec:lower}, we give an example of a $(2k +2)$-wise independent
distribution where $\E[|S_\ell|]$ for $\ell \in \{2k +3,\ldots, n- 2k
-3\}$ is much larger than under the uniform distribution. This shows
that one can only hope to show tail bounds for larger $\ell$. The same
example also shows that our tail bounds are close to tight.

%Our approach for showing these  follows
As discussed earlier, \cite{GMRTV} require a bound on higher moments
of the variables. More precisely, they assume that 
\begin{align*}
\E[X_i^{2k}] \leq (2k)^{2k}\sigma_i^{2k}
\end{align*}
for all $i \in [n]$.
They additionally require $\sigma =o(1)$ as opposed
to being bounded by some constant. Bounding the higher moments introduces technical difficulties and case analyses in their
proofs. In contrast, bounding the second moments (as we require here) is immediate. 
Theorem~\ref{thm:main} can be used to simplify their proofs. 


In place of Theorem \ref{thm:boundUsingS1E2}, one could plug in the bound given by Equation
\eqref{eqn:GMR} \XX{to} get a somewhat weaker version of Theorem \ref{thm:GenBound}.  
However, it seems that the resulting bound will not be
strong enough to prove Theorem \ref{thm:main}, and the asymptotic
improvement given by Theorem \ref{thm:boundUsingS1E2} is crucial.



Our stronger result is obtained by replacing the usual
Inlcusion-exclusion based expansion in Equation \eqref{eq:incl-excl}
with a Taylor-series style expansion about the mean, as in \cite{GMRTV}. Let
$X_i = \mu(1 + Z_i)$ where $\E[Z_i] = 0$ and $\E[Z_i^2] =
\sigma_i^2/\mu_i^2$. We have
\begin{align}
\label{eq:taylor}
\E[\prod_{i=1}^nX_i] = \E[\prod_{i=1}^n\mu_i(1+ Z_i)] = \prod_{i=1}^n\mu_i\left( \sum_{k=0}^n\E[S_k(Z_1,\ldots,Z_n)]\right).
\end{align}
It is easy to show that the $\E[|S_k(Z_1,\ldots,Z_n)|] \leq
\frac{\sigma^k}{\sqrt{k!}}$. If $|S_k(Z_1,\ldots,Z_n)|$ were to give a bound on the error
after truncating the series to $k$ terms, we would be done. However,
this need not be true. Note that the $Z_i$s can take on negative values, so the
inclusion-exclusion formula does not apply. Further, while the
expectations of the higher degree polynomials are well bounded under the
uniform distribution, it seems hard to control them assuming just $k$-wise
indpendence.


We use this to show that even though we cannot bound $\E[S_\ell(Z_1,\ldots,Z_n)]$ under $k$-wise
indpendence once $\ell \gg k$, we can still get strong tail bounds on
them. This lets us show that truncating Equation \eqref{eq:taylor}
after $k$ terms gives error roughly $O(\sigma^k)$, and thus $k =
O(\log(1/\delta)/\log(1/\sigma)$ suffcies to get error $\delta$.






\eat{
}

